SchedCheck: Schedule-Robustness Analysis for Event-Driven Block Programs

Block-based languages such as Scratch let beginners assemble interactive programs from sprites and scripts. These programs are concurrent in practice: green-flag scripts, broadcasts, and clones run as cooperatively scheduled threads over shared sprite and stage state, and their authors never write a thread. We show that such programs contain schedule-sensitive behaviors whose observable result depends on an execution order the language leaves open. Editing, saving, or remixing a project can produce a copy with the same blocks but a different layer order, changing the order the virtual machine starts scripts. We formalize the schedule space a Scratch virtual machine can realize as the permutations of the initial executable-target order, and define schedule-robustness against a lattice of observation lenses over a fixed horizon. A partial-order exploration runs one schedule per dependence-equivalence class, and on projects small enough to enumerate, an independent oracle confirms it recovers every realizable outcome. On larger projects, representatives stand in for the factorial under the validated dependence model. SchedCheck implements this on the production Scratch VM. Across 224 real student projects, at least 21% of the concurrent ones are schedule-sensitive at the grading lens, and a uniform random sample of public projects replicates the rate at 17.6%, with two real remixes of a deployed animation arranging its letters differently. On hand-built fault pairs and a generated benchmark of 32 spec-defined faults across four classes, the tool detects and localizes every schedule fault, with a logic-fault control reporting clean. The oracle exposed four unsoundness gaps in the dependence model, all repaired. The method is parametric in the execution model, instantiating unchanged on a second cooperative event loop.

==> sec-overview.tex <==
\section{Overview}
\label{sec:overview}

\sys{} answers one question: can a sprite-order change alter what a project does? A run is fixed once the input, the seed, and the sprite order are set, and the order is the only one a user controls without editing blocks. The realizable orders permute the sprites, each from a layout the editor can produce, and the ball-and-paddle project of Figure~\ref{fig:example} has two that give the counter two values. A harness pins the seed, clock, and identifier allocation, so a difference is the order's doing and a witness reruns on the stock VM. \sys{} reads each run through a lens, runs one representative per group of orders that must agree, checks the grouping against an exhaustive run wherever a project is small enough, and turns a difference into the two scripts that contend for a resource. The sections that follow give the schedule space (Section~\ref{sec:model}), the testing loop (Section~\ref{sec:testing}), the two algorithms and the oracle (Section~\ref{sec:dpor}), and the evaluation (Section~\ref{sec:eval}).

